Program Synthesis Over Noisy Data with Guarantees

We explore and formalize the task of synthesizing programs over noisy data, i.e., data that may contain corrupted input-output examples. By formalizing the concept of a Noise Source, an Input Source, and a prior distribution over programs, we formalize the probabilistic process which constructs a noisy dataset. This formalism allows us to define the correctness of a synthesis algorithm, in terms of its ability to synthesize the hidden underlying program. The probability of a synthesis algorithm being correct depends upon the match between the Noise Source and the Loss Function used in the synthesis algorithm's optimization process. We formalize the concept of an optimal Loss Function given prior information about the Noise Source. We provide a technique to design optimal Loss Functions given perfect and imperfect information about the Noise Sources. We also formalize the concept and conditions required for convergence, i.e., conditions under which the probability that the synthesis algorithm produces a correct program increases as the size of the noisy data set increases. This paper presents the first formalization of the concept of optimal Loss Functions, the first closed form definition of optimal Loss Functions, and the first conditions that ensure that a noisy synthesis algorithm will have convergence guarantees.

==> design.tex <==



==> incorrecttable.tex <==
\begin{figure}
\begin{center}
\begin{tabular}{|l|c|c |c|}
\hline
    \multirow{2}{*}{Benchmark} & \multirow{2}{*}{Data Set} & \multicolumn{2}{c|}{Number of Required} \\
    \multirow{2}{*}{} & \multirow{2}{*}{Size} & \multicolumn{2}{c|}{Correct Examples} \\
    \cline{3-4}
    & & 1-Delete&DL\\
\hline
    bikes & 6 &0& 0 \\
    dr-name & 4& 0&0 \\
    firstname & 4&0& 0 \\
    lastname & 4& 0& 2 \\ %Look into this
    initials & 4& 0& 2 \\
    reverse-name & 6 & 0& 0 \\
    name-combine & 4& 0& 0 \\
    name-combine-2 & 4 & 0& 0 \\
    name-combine-3 & 4 & 0& 0 \\
    phone & 6 & 0& 2 \\
    phone-1 & 6 & 0& 3 \\
    phone-2 & 6& 0& 2 \\
    phone-5 & 7 & 0& 2 \\
    phone-6 & 7 & 0& 2 \\
    phone-7 & 7 & 0& 2 \\
    phone-8 & 7 & 0& 0 \\
\hline
\end{tabular}
\end{center}
\vspace{-.1in}
    \caption{\TODO{Rerun}
        Minimum number of correct examples required to synthesize correct a program.}
    \label{table:minexample}
\vspace{-.2in}
\end{figure}



==> metrics.tex <==
\section{Loss function Metrics}
Given the noisy program synthesis framework 
(Section~\ref{})
and the underlying statistical
program synthesis theory (Section~\ref{}), we connect this through formalizing
the quality of a Loss Function via quality metrics. 


Given data set $\cD = (\vec{x}, \vec{y})$, DSL $G$, program probability $\pi$,
our synthesis algorithm finds a program $p^*$, such that 
\[
    p^* = \arg \min_{p \in G} \cL(p, \cD) - \log \pi(G)
\]


We use the following notation within this section,
\[
    \cE(\cL~\vert~\vec{x}, \vec{y}) = \cE(\vec{z}_{\cL}~\vert~\vec{x}, \vec{y}) 
\]
where $Z_{\cL, \pi} = \inf_{Z \in G[X]} \cL(\vec{z}, \vec{y}) - 
\log \pi(\vec{z}~\vert~\vec{x})$, and $G[\vec{x}] = \{
    \vec{z}~\vert~\vec{z}=p[\vec{x}]\}$.




\subsection{Correctness Metrics}
We first, formalize how correct a program is with respect to given loss
function.


Given an input set $\vec{x}$ and noisy output set $\vec{y}$, we quantify how correct a loss
function is with respect to underlying probability distributions.

\begin{definition}[\bf Correctness]
    Given an input set $\vec{x}$, and noisy dataset $\vec{y}$, a loss function $\cL$
is correct if and only if 
\[
    \inf_{\vec{z} \in G[\vec{x}]} \cL(\vec{z}, \vec{y}) - 
    \log \pi(\vec{z}~\vert~\vec{x}) = 
    \inf_{\vec{z} \in G[\vec{x}]} \cE(\vec{z}~\vert~\vec{x}, \vec{y})
\] 
i.e. output set which minimizes the loss function, also minimizes the expected
risk.
\end{definition}

\begin{definition}[\bf Reflexive Correctness]
    Given a DSL $G$, an input set $\vec{x}$, loss function $\cL$,  is reflexive correct 
    if for all programs $p \in G$, $\vec{z}_p = p[\vec{x}]$, 
\[
    \vec{z}_p = \inf_{\vec{z} \in G[\vec{x}]} \cL(\vec{z}, \vec{z}_p) - \log
    \pi(\vec{z}~\vert~\vec{x})
\] 
\end{definition}


\begin{definition}[\bf Expected Correctness]
\end{definition}



Robustness, Given $X$, measures how much tolerance the loss function has to
still get us the same answer.

\begin{definition}[\bf $Z$-Robustness]
    \[
        a 
    \]
\end{definition}


Min of Robustness over all programs

\begin{definition}[\bf Robustness]

\end{definition}


The consistency`


\begin{definition}[\bf $n, k$-Consistency]
    Let $X = \tup{x_1, \ldots x_n}$, $X' = \tup{x_1, \ldots x_n, 
    x_{n+1} \ldots x_{n_k}}$, $\cY = \tup{y_1, \ldots y_n}$, and .

    \[
        \cR(\cL~\vert~X, X') = P(Z \leq Z'~\vert~Y \leq Y') 
    \]
\end{definition}

\begin{definition}[\bf Consistency]

\end{definition}



increase $X$ and then see if $Z^*$ improves

$Pr(\cE(L) - \inf \cE() < \epsilon) > 1 - \delta$



